Prototype-based Incremental Few-Shot Semantic Segmentation

Semantic segmentation models have two fundamental weaknesses: i) they require large training sets with costly pixel-level annotations, and ii) they have a static output space, constrained to the classes of the training set. Toward addressing both problems, we introduce a new task, Incremental Few-Shot Segmentation (iFSS). The goal of iFSS is to extend a pretrained segmentation model with new classes from few annotated images and without access to old training data. To overcome the limitations of existing models iniFSS, we propose Prototype-based Incremental Few-Shot Segmentation (PIFS) that couples prototype learning and knowledge distillation. PIFS exploits prototypes to initialize the classifiers of new classes, fine-tuning the network to refine its features representation. We design a prototype-based distillation loss on the scores of both old and new class prototypes to avoid overfitting and forgetting, and batch-renormalization to cope with non-i.i.d.few-shot data. We create an extensive benchmark for iFSS showing that PIFS outperforms several few-shot and incremental learning methods in all scenarios.

==> sec/method_sett.tex <==
\begin{table}[t]
\centering
    \setlength{\tabcolsep}{20pt} % Default value: 6pt
    \resizebox{\linewidth}{!}{
\begin{tabular}{l|c c c c c}
                        \multirow{2}{*}{Semantic Segmentation}&       \multicolumn{2}{c}{Training}    &   \multicolumn{2}{c}{Output}  \\ 
                        & data & few-shot& class& multi-step\\\hline
                        Offline &$\set D^0$& -&$\set C^0$& - \\
                         \hline
Few-Shot     \cite{shaban2017one, rakelly2018few, dong2018few, zhang2019canet}         & $\set D^{t}$  &    \cmark &$\set K^t$  & - 
\\
Generalized Few-Shot  \cite{xian2019spnet}& $\cup_{s=0}^{t}\set D^{s}$  & \cmark& $\set C^t$& - \\
Incremental Learning \cite{michieli2019incremental,cermelli2020modeling}& $\set D^t$&-&$\set C^t$&\cmark\\\hline
\textbf{Incremental Few-Shot}     & $\set D^t$  &\cmark&  $\set C^t$   & \cmark \\
\end{tabular}}
\vspace{-5pt}
\caption{Comparing different semantic segmentation settings. $t$ denotes the current learning step, $\set K^t$ denotes all classes labeled in $\set D^t$ while $\set C^t=\cup_{s=0}^{t}\set K^{s}$.} 

\label{tab:setting-comparison}
\vspace{-15pt}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/method-crop.pdf}\vspace{-5pt}
    \caption{Illustration of \ours. {In the base step (top left), we train a prototype-based model using the cross-entropy loss $l_{CE}$.} Then (top right), given few images of a new  class, we initialize its prototype with %update the classifier using 
    Masked Average Pooling (MAP). We then fine-tune the network using the CE loss and our prototype-based knowledge-distillation ($l_{KD}$) to preserve old knowledge while reducing overfitting the new class representation (bottom). To cope with the non-\textit{i.i.d.} few-shot data, we use batch-renorm in place of batch-norm in the few-shot learning steps.} 
    \label{fig:method}
    \vspace{-15pt}
\end{figure}

\section{Prototype Learning for iFSS} \label{sec:method}
In this section, we define the novel Incremental Few-Shot Segmentation (\SET) setting and we method able to cope with its challenges: \textit{\oursFull} (\ours). 
\ours\ uses prototype learning to learn class prototypes and effectively integrate new classes from few-shots. In the few-shot learning (FSL) step, the model is trained end-to-end to improve the network representation, reducing both forgetting and overfitting with a prototype-based distillation loss.
Figure \ref{fig:method} gives an overview of the approach.

%\myparagraph{Problem Definition.} 
\subsection{Incremental Few-Shot Segmentation (\SET)}  \label{sec:setting}
The goal of \SET\ is to learn a model that assigns to each image pixel its corresponding semantic label in a set $\set C$. Differently from standard semantic segmentation, $\set C$ is expanded over time using few images with pixel-level annotations of the new classes. 

Formally, let us denote as $\set C^t$ the set of semantic categories known to the model after learning step $t$, where \textit{learning step} denotes and update of the model's output space. During training we receive a sequence of datasets $\{\set D^0, \dots, \set D^T\}$ where $\set D^t = \{(x, y)| x \in \set X\,, y \in \set Y^t\}$. In each $\set D^t$, $x$ is an image in the images space $\set X\in \real^{|I|\times 3}$, where $I$ is the set of pixels, and $y$ its corresponding label mask in $\set Y^t \subset \set (C^t)^{|I|}$. Note that $\set D^0$ is a large dataset while $\set D^t$ are few-shot ones, \ie $|\set D^0|\gg|\set D^t|$, $\forall t\geq1$. The model is first trained on the large dataset $\set D^0$ and % containing pixel level annotations for several semantic categories. Then, i
incrementally updated with few-shot datasets. % $\set D^t$ is available. 
We name the first learning step on $\set D^0$ as the \textit{base} step. 
Note that at step $t$ the model has access only to $\set D^t$. %, with $\set C^0$ as the base classes. 
 % This implies that at learning step $t+1$ we have access only to the dataset $\set D^{t+1}$.

From the formulation, we make two assumptions: i) each dataset contains annotations for new classes, \ie $\set C^t \subset \set C^{t+1}$; ii) pixels of old classes $\set C^t$ will be labeled in $\set D^{t+1}$ if present. %, since annotating few images is cheap. 
\fabio{Note that annotating few images is cheap, in contrast to \cite{cermelli2020modeling} where the dataset $\set D^{t+1}$ is large and annotating all the classes is expensive}.
% Note that we do not require that $\set D^{t+1}$ contains classes in $\set C^t$. 
Differences between \SET\ and existing settings are summarized in \tabref{tab:setting-comparison}.%, we will have no pixels and labels of classes in $\set C^t$.
%{We will refer to $\set C^0$ as \textit{Base} classes, and to $\set C^t \backslash \set C^0$ as the \textit{New} ones.}

 
% % \fabio{Should we mention Incremental Few-Shot learning and detection \cite{perez2020incremental, gidaris2018dynamic, tao2020few}?}
% \myparagraph{Difference with Few-shot Learning.}
% %Despite requiring the capability to segment new objects given just few-annotated images, we want to highlight that 
% Despite learning to segment objects from few images, \SET\ differs from previous few-shot segmentation settings \cite{shaban2017one, rakelly2018few, dong2018few, zhang2019canet, wang2019panet, siam2019adaptive} since %In particular, we do not restrict the output space of the model to the set of new classes. 
% %Denoting as $\set K^t$ the set of classes with at least one annotated pixel in the set $\set D^t$, \ie $\set K^t = \{k | k\in C^t \wedge \exists y \in \set D^t : y_i=k\}$, where $y_i$ denotes the label of pixel $i$ in $y$. 
% they limit the output space to the new classes labeled in $\set D^t$, discarding previous knowledge. In \SET\ the output space contains all classes and can be  %, \ie $\set C^t = \bigcup_{s=0}^{t-1} \set K^s$,
%  expanded over time.

% \myparagraph{Difference with Generalized Few-shot.}
% \SET\ and Generalized Few-Shot Segmentation \cite{xian2019spnet} share the same goal, \ie %. The goal of the two tasks is the same \ie 
% segmenting both base and new classes. However, in \SET\ at learning step $t$ we have access only to $\set D^t$ while in GFSS to all datasets, \ie  $\set D_{\text{GFSS}}^t = \bigcup_{s=0}^t \set D^s$. %Storing all datasets %has the drawback of i) requiring longer training procedures (\ie spanning the union of all datasets) and ii) 
% %is unfeasible in scenarios with %old data cannot be stored for \eg 
% %memory constraints. 
% Without previous datasets, we may experience catastrophic forgetting \cite{mccloskey1989catastrophic}. 

% \myparagraph{Difference with Incremental Learning.}
% As in incremental learning for semantic segmentation \cite{michieli2019incremental, cermelli2020modeling}, the goal of \SET\ is to expand the output space of the model without access to previous datasets, avoiding catastrophic forgetting. However, in IL we add new knowledge from large datasets, while in \SET\ we use just few images per class. %, while in IL with large datasets. %\SET\ poses the challenge of learning a classifier for the new classes from few samples while avoiding forgetting.  

\subsection{Prototype Learning}
\label{sec:proto-init} 
\myparagraph{Learn a prototype-based model.}
Our goal is to learn a model $\phi^t$ that maps each pixel to a probability distribution over the set of classes, \ie $\phi^t : \set X \to \real^{|I|\times |\set C^t|}$, where $t$ denotes the last learning step. 
We assume $\phi^t$ made of a feature extractor $f^t: \set X \to \real^{|I|\times d}$ and a classifier $g^t: \real^{|I|\times d}  \to \real^{|I|\times |\set C^t|}$, so that $\phi^t = g^t \circ f^t$. Here, $d$ is the feature dimension and $g^t$ is a softmax classifier with parameters $W^t = [w^t_1, \dots, w^t_{|\set C^t|}] \in \real^{d \times |\set C^t|}$. %Note that state-of-the-art segmentation architectures \cite{chen2017deeplab, zhao2017pyramid} fit in this definition. 

In the base step, we want to prepare $\phi^0$ to include new classes given few examples. %To this end, we need our model to i) extract as much information as possible from the few available images while ii) avoiding biases toward either old or new classes. 
To this aim, we enforce the classifier weights to represent class prototypes. The prototypes shall reflect the average pixel-level features of a class, so that the features extracted from (few) pixels of the new classes provide a good estimate of %used to directly initialize 
their corresponding classifier weights. Following previous works \cite{gidaris2018dynamic, qi2018low}, we achieve this through a cosine classifier. 

Formally, in the base %learning 
step, we train the network with a cross-entropy loss over all pixels: %the pixel-level class scores: %cosine similarities among each feature vector and the class prototypes:
\begin{equation}
\label{eq:objective}
    \ell^0_{CE}(x,y) = -\frac{1}{|I|} \sum_{i \in I} \log \phi_{y_i,i}^0(x)
\end{equation}
where $\phi_{c,i}^0(x)$ is the probability of pixel $i$ of $x$ to belong to class $c$. The score $\phi_{c,i}^t(x)$ % for a class $c$ in pixel $i$ 
is computed as a softmaxed cosine similarity between the features and the class prototype $w^t_c$:
\begin{align}
    \phi_{c,i}^t(x) = g_{c,i}^t(f^t(x)) = \frac{e^{s_{c,i}^{t}}}{\sum_{k \in \set C_0} e^{s_{k,i}^{t}}}, \;\;\;    s_{c,i}^{t} = \tau \frac{f_i^t(x)^\intercal  w^t_c}{||f_i^t(x)||\ ||w^t_c||}
\end{align}
where %$w^t_c$ being the classifier weight for class $c$, 
$f_i^t(x)$ are the features extracted at pixel $i$, and $\tau$ is a scalar which scales the similarity in the range $[-\tau, \tau]$. 
With the cross-entropy loss in Eq.~\eqref{eq:objective}, the model minimizes the cosine distance between a prototype and the features of a given class,  % and the prototype of the ground-truth class. As a consequence, the classifier 
capturing the compatibility between feature vectors and class prototypes.

\myparagraph{Initialize prototypes of new classes.}
% We need to first initialize the classifier's parameters for each new class in $K^t$. Since the objective in \equref{eq:objective} ensures that the classifier weights represent class prototypes, we can 
Given a dataset $\set D^t$, let us denote as $\set K^t$ the set of new classes, \ie $\set K^t = \set C^t \setminus \set C^{t-1}$. After the base step, we can initialize the parameters for each $k\in\set K^t$ as their respective prototypes, performing \textit{weight imprinting} \cite{qi2018low}. Since we know that features of a class $k$ provide an estimate of the prototype $w_k$, we can compute the new class prototypes by aggregating the set of features extracted for each pixel of the class $k$ in $\set D^t$. % corresponding to each pixel $i$ of a class $k$ in each new image $x \in \set D^t$. 
Inspired by \cite{siam2019adaptive, dong2018few, wang2019panet}, we use masked average pooling: 
%MAP consists in computing the  average of all the feature vectors in $\set F_k^t$ corresponding to pixels of the class of interest $k$. Given the set $\set D^t$, 
%We compute MAP for class $k$ as:
\begin{equation}\label{eq:map}  w^t_k = 
    \text{MAP}_k({\set D^t}) = \frac{1}{|\set D^{t}_k|}\sum_{(x,y) \in \set D^{t}_k}\frac{\sum_{i \in I} M_{k,i}(y) \frac{f^t_i(x)}{||f^t_i(x)||}}{\sum_{i \in I} M_{k,i}(y)}, 
\end{equation}
where $M_{k}(y)$ is a binary mask indicating which pixels belong to class $k$ and $\set D^{t}_k$ is the set of images in $\set D^t$ containing at least one pixel of class $k$. As we will show experimentally, this strategy provides a good initial estimate of the classifier that is not needed in standard IL but is crucial in \SET\ for learning to segment new classes from few samples. 
%The MAP can be directly employed as the classifier weights of each new class $k \in \set K^t$, \ie $w^t_k = \text{MAP}_k({\set D^t})$.

\subsection{Distilling Prototypes for \SET}

%As we will show experimentally, and witnessed by previous works \cite{qi2018low, gidaris2018dynamic}, WI is a general strategy for few-shot learning, whose effectiveness is independent on the particular setting and task. However, 
Although weight imprinting is a good classifier initialization strategy, relying on a feature extractor tuned on different semantic classes (\ie $\set C^{t-1}$) is suboptimal. %, due to the limited since the ability of the network to extract good features for unseen classes is limited. 
To refine the network representation, we train the model \textit{end-to-end} in the few-shot learning steps. As pointed out in \cite{gidaris2018dynamic,perez2020incremental}, end-to-end training in FSL steps may lead to overfitting and forgetting. %\cite{gidaris2018dynamic} and forgetting %old knowledge
%\cite{perez2020incremental}. %However, while na\"ive end-to-end training would produce poor results,
We address these issues %borrowing ideas from the IL literature. In particular, we propose to use  
designing a distillation loss on the prototypes that regularizes the training and reduces both overfitting and catastrophic forgetting. We also use batch-renormalization to cope with the non-\textit{i.i.d}. few-shot data. In the following we describe the two components. %The ideal solution would be to fine-tune the network on new class data. However, 
% previous works \cite{gidaris2018dynamic, perez2020incremental} point out that fine-tuning should not be performed on incremental few-shot  
% since it is prone to (i) over-fitting the new classes, due to the limited amount of data \cite{gidaris2018dynamic}
% , and (ii) catastrophic forgetting \cite{mccloskey1989catastrophic}, since without revisiting the data for previous knowledge the network is biased toward new data \cite{perez2020incremental}. Here we take a different perspective and we argue that end-to-end training on few-shot network can largely boosts the performance of the model. This is possible if i) we keep into account the incremental nature of the task, borrowing principles of IL to avoid catastrophic forgetting and ii) we devise a strategy to address the shift in the data distributions caused by the non i.i.d. few-shot samples. 

\myparagraph{Prototype-based Distillation.} %We start by describing how we design our end-to-end training objective for every few-shot learning step $t$, with $t\geq1$. In this scenario, 
Given a pair $(x,y)\in \set D^t$, we update $\phi^t$ by minimizing: % the following loss function:
\begin{equation}
\label{eq:objective-few-shot}
    \ell^t(x,y) = \ell^t_{CE}(x,y) + \lambda \ell^t_{KD}(x, \phi^t,\phi^{t-1})
\end{equation}

where $\lambda$ is a trade-off hyperparameter, $\ell^t_{CE}$ is the cross-entropy loss of Eq.~\eqref{eq:objective} over $\set C^t$ and $\ell^t_{KD}$ is a knowledge distillation loss where %a regularization objective and $\lambda$ is a trade-off between the two. In the IL literature, multiple choices have been explored for $\ell^t_{R}$, ranging from parameter-driven objectives \cite{kirkpatrick2017overcoming, chaudhry2018riemannian} to knowledge distillation \cite{li2017learning,michieli2019incremental,cermelli2020modeling}. Here we follow the latter strategy. In particular, 
$\phi^{t-1}=g^{t-1}\circ f^{t-1}$ is a copy of the network after the previous learning step. The old model $\phi^{t-1}$ acts as a teacher and the current model $\phi^t$ as a student, minimizing the objective:
\begin{equation}
    \label{eq:kd-general}
    \ell^t_{KD}(x, \phi^t,\phi^{t-1})  = \frac{1}{|I|} \sum_{i \in I} d(x_i, \phi^{t-1}, \phi^{t})
\end{equation}
where $d$ is a general distance function. Minimizing the objective in Eq.~\eqref{eq:kd-general} forces the model to extract representations that do not deviate from the discriminative ones for the old knowledge, reducing catastrophic forgetting. While previous works in IL %for semantic segmentation 
instantiate $d$ as either L2 at the feature-level \cite{michieli2019incremental}, or cross-entropy on the probabilities of old classes \cite{cermelli2020modeling}, here we fully exploit the good initialization given by the prototype-based classifier. In particular, we define as $\hat{\phi^{t}} = \hat{g}^t \circ f^{t-1}$ the network whose classifier weights $\hat{W}^t$ of $\hat{g}^{t}$ for class $k\in \set K^t$ are initialized as in Eq.~\eqref{eq:map}, %\ie:
% \begin{equation}
% \hat{w}_k^t = 
% \begin{cases}
% w^{t-1}_k,   &\text{if} \;k \in \set C^{t-1}\\
% \text{MAP}_k({\set D^t}) & \text{otherwise.}
% \end{cases}
% \end{equation}
\fabio{and our distance function as:}
\begin{equation}\label{eq:self-distill}
    d(x, \phi^t, \hat{\phi}^t) = -\sum_{c\in\set C^t} \hat{\phi}_c^t(x)\log \phi_c^t(x).
\end{equation} 
In Eq.~\eqref{eq:self-distill}, we explicitly consider the scores that the old network representation produces for both old classes in $\set C^{t-1}$ and \textit{new} ones in $\set K^t$. This forces the model to keep scores for old classes similar to the old model, and encourages the prototypes of new classes to be close to their initial estimate given by $f^{t-1}$. %In fact, forces $\phi^t$ to not deviate from the old feature extractor (since prototypes are initialized from $f^{t-1}$) while reducing overfitting on local information of the few-shot dataset by forcing coherence with the . %. The latter follows the principle of \textit{refining} the model for new classes % where the latter is obtained through the classifier initialized with weight imprinting. 
The advantage of this new formulation \wrt standard knowledge distillation in IL \cite{michieli2019incremental,cermelli2020modeling,rebuffi2017icarl,li2017learning} is that we address catastrophic forgetting %of old knowledge 
while reducing overfitting %the risk to overfit the model 
on the few-shot data of new classes, % the representation and classifier learned for new classes, 
a main problem in \SET. 

\myparagraph{Coping with non i.i.d. data.}
Despite the regularized training, we found that in extreme few-shot scenarios (\eg 1-shot settings) a main cause of the drop in performance is the drift of statistics in the batch-normalization (BN) \cite{ioffe2015batch} layers of the network. BN assumes independent and identically distributed (\textit{i.i.d.}) data \cite{ioffe2015batch, ioffe2017batch} but in the FSL steps we have small datasets where most pixels belong to new classes, thus the input is inherently non \textit{i.i.d.}. Updating the statistics on this non-\textit{i.i.d.} set makes them poor and biased.

Two simple solutions are either using %to normalize the FSL data either with 
the global BN statistics of the base step, % on $\set D_0$, 
or the training batch ones but without updating their global estimate used at test time. However, we found the first solution causing training instability and the second poor performance due to misalignment between features extracted for the new classes at training and test time. %without normalizing the features during training we found that the gradients explode, making end-to-end training unfeasible. Another solution may be to freeze the BN statistics during inference but not during the FSL step. However, this solution does not bring improvements since the network will be trained using the (non \textit{i.i.d.}) batch statistics, which differ from the ones collected in the initial training stage, thus introducing a misalignment between features extracted for the new classes between training and test time. 

Ideally, we want to normalize features in the FSL step while i) avoiding the shift of the statistics toward the new class data and  ii) aligning training and inference statistics. % with the inference ones. %, as extracted by the main architecture. 
To achieve this, we take inspiration from continual learning works with non-i.i.d. data \cite{lomonaco2020rehearsal} and use
Batch Renormalization (BR) \cite{ioffe2017batch}.
% In practice, BN layers normalize each value of the input $z^c_i$, where $c$ indicates the channel and $i$ its spatial position, to have a learnable mean and standard deviation:
% \begin{equation}
%     \hat{z}^c_i = \gamma \frac{z^c_i - \mu^c}{\sigma^c} + \beta,
% \end{equation}
% where $\gamma$ and $\beta$ are the learnable parameters, and $\mu^c$ and $\sigma^c$ are, respectively, the mean and standard deviation across all the images in the batch on the channel $c$. 
% During inference, the BN layers replace the batch statistics with the running statistics, which are the moving averages of the mean $\mu^c_r$ and standard deviation $\sigma^c_r$:
% \begin{equation}
%     \hat{z}^c_i = \gamma \frac{z^c_i - \mu^c_r}{\sigma^c_r} + \beta.
% \end{equation}
Batch Renormalization (BR) revisits BN by normalizing a feature $q$ with the running statistics in place of the training batch statistics:
\begin{equation}
    \hat{z}^q_i = \gamma (\frac{z^q_i - \mu^q}{\sigma^q} \frac{\sigma^q}{\sigma_r^q} + \frac{\mu^q - \mu^q_r}{\sigma_r^q}) + \beta,
\end{equation}
where  $\gamma$ and $\beta$ are learnable parameters,  $\mu_r^q$ and $\mu^q$ the global and batch mean, and $\sigma_r^q$ and $\sigma^q$ the global and batch standard deviation. %and global one and $\sigma^c$, are, respectively, the mean and standard deviation across all the images in the batch on the channel $c$. It is important to note that the gradient does not flow in $r$ and $d$, so the normalization effect on the gradient is still active. 
We freeze $\mu_r^q$ and $\sigma_r^q$ after the base step to prevent them from shifting toward new classes and damaging the performance on base ones. %As we will show experimentally, this simple change is crucial to perform stable end-to-end training in the FSL step.  

% Replacing BN layers with BR ones in the few-shot learning steps ensures that features of new classes are normalized with the same statistics both during training and inference. Additionally, by freezing the statistics we avoid that they get shifted toward new classes, preventing a drastic decrease in performance on old classes. At the same time, BR retains the same benefits of BN (\ie avoiding exploding gradients), which is fundamental for end-to-end training. 
































==> sec/name.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{6pt} % Default value: 6pt
%\resizebox{\linewidth}{!}{
\begin{tabular}{rc||cc|c||cc|c||cc|c|}
            &  & \multicolumn{3}{c}{1-shot} & \multicolumn{3}{c}{2-shot} & \multicolumn{3}{c}{5-shot} \\
            & train & Base  & Novel  & Harm    & Base  & Novel   & Harm  & Base  & Novel & Harm   \\ 
WI         & - & \textbf{66.7}  & \textbf{14.2}   &	\textbf{23.5}	& \textbf{67.7}	& \underline{17.5}  & \underline{27.8}  & \textbf{67.5}  & 18.4  & 28.9       \\ \hline
FT          & $g$ & 60.9  &  9.6   &	16.6	& 60.8	& 15.7	  & 25.0  & 59.3  & 20.4  & 30.3   \\
%COS         & $g$ & 61.6  &  7.5   &	13.3	& 62.9	& 11.5	  & 19.5  & 63.9  & 16.0  & 25.6   \\
%WIT         & $g$ & 61.7  &  8.5   &	15.0	& 62.8	& 12.9	  & 21.5  & 64.2  & 18.7  & 29.0   \\ \hline
FT          & $\phi$ & \underline{62.4}  &  6.3   &	11.5	& \underline{62.5}	& 15.0	  & 24.2  & 62.0  & \underline{23.0}  & \underline{33.5}     \\
%COS         & $\phi$ & \underline{63.3}  &  7.5   &	13.5	& \underline{64.4}	& \underline{18.4}	  & \underline{28.6}  & \underline{65.9}  & \textbf{29.6}  & \textbf{40.9}     \\
WIT         & $\phi$ & 61.4  &  \underline{9.9}   &	\underline{17.1}	& 61.2	& \textbf{20.9}	  & \textbf{31.2}  & \underline{62.7}  & \bf{28.6}  & \bf{39.3}
\end{tabular}%}
\caption{Comparison of fine-tuning strategy on the Pascal-VOC \cite{pascal-voc-2012}. Best in \textbf{bold}, second best \underline{underlined}} %\zeynep{cite the WI in the table}.\fabio{The issue is that WI is not easily linked to a paper, is a general idea we adapted to segmentation}}
\label{tab:training-ablation}
\end{table*}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\resizebox{\linewidth}{!}{
\begin{tabular}{r||cc|c||cc|c|}%|cc|c|}
\multicolumn{1}{l}{}  & \multicolumn{3}{c}{1-shot} & \multicolumn{3}{c}{2-shot} \\ %& \multicolumn{3}{c}{5-shot} \\
            & Base    & Novel   & Harm   & Base    & Novel   & Harm \\ % & Base    & Novel   & Harm  \\
WI          & \textbf{66.7}    &	14.2 &	23.5  & \textbf{67.7}	& 17.5	  & 27.8 \\ % &	67.5    & 18.4    & 28.9  \\
FT          & {62.4}  &  6.3   &	11.5	& {62.5}	& 15.0	  & 24.2 \\ \hline
WIT         & 61.4    &	 9.9 &	17.1  & 61.2	& 20.9	  & 31.2 \\ \hline % &	62.7    & 28.6    & 39.3  \\ \hline
WIT+BR      & 64.0    &	{16.8} &	{26.6}  & 62.4	& {23.8}	  & {34.4} \\ % & 61.4	& 30.2	  & 40.5  \\
WIT+BR+L2   & \textbf{66.7}    & \textbf{17.4}    & \textbf{27.6}   & {66.0}    & \textbf{24.7}    & \textbf{36.0}  \\ % & 64.7    & 32.0    & 42.8   \\

\end{tabular}}
\end{table}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\resizebox{\linewidth}{!}{
\begin{tabular}{r||cc|c||cc|c|}
        & \multicolumn{3}{c}{1-shot} & \multicolumn{3}{c}{2-shot}\\ % & \multicolumn{3}{c}{5-shot} \\
    & Base    & Novel   & Harm   & Base    & Novel   & Harm  \\\hline % & Base    & Novel   & Harm   \\
WIT+BR      & 64.0    & 16.8    & 26.6   & 62.4    & 23.8    & 34.4  \\  % & 61.4    & 30.2    & 40.5   \\
\end{tabular}}
\caption{The effect of regularization loss to avoid forgetting.}
\label{tab:ablation-reg}
\end{table}

==> sec/related.tex <==

\section{Related Works}

\vspace{-4pt}\myparagraph{Semantic Segmentation.}
%Modern  architectures \cite{long2015fully, chen2018encoder, zhao2017pyramid, lin2017refinenet, zhang2018exfuse} enabled great progress in semantic segmentation. 
State-of-the-art semantic segmentation models use a fully convolutional encoder-decoder networks \cite{long2015fully, badrinarayanan2017segnet}, integrate % differ on how they integrate 
contextual information on pixel-level features in different ways, e.g. through %. There are two main approaches: 
pyramids %, using multiple input scales 
\cite{zhao2017pyramid,lin2017refinenet,chen2017rethinking, chen2017deeplab, zhang2018exfuse, chen2018encoder}, %that integrate modules exploiting information at different scales, 
or attention \cite{yu2020context, yuan2019object, yu2018learning, yuan2018ocnet, fu2019dual, zhang2018context}. % aggregates the long-range spatial dependencies using attention modules at different levels.
These models need a large dataset for training, which is often expensive to collect, and they only consider an offline setting, with a static output space. % where the output space of the model is fixed after training. %, \ie after the model is trained, its output space is fixed. % and no addtional . 
Here we address both issues, extending the output space of a model using just a few annotated images.
%\fabio{Should we talk about weakly supervised and zero-shot learning?}

% \myparagraph{Few-Shot Learning.}
% \fabio{
% % tre tipo di lavori: meta-learning, metric-learning, hallucination based.
% Few-shot learning (FSL) has been studied extensively in image classification \cite{snell2017prototypical, koch2015siamese, finn2017model, hariharan2017low, gidaris2018dynamic, tian2020rethinking, sung2018learning} and has the goal to learn to classify novel classes, given only few images depicting them, starting from an abundant labeled dataset of base classes. There most common approaches for FSL meta-learn a network and can be divided in metric-learning based meta-learning \cite{snell2017prototypical, koch2015siamese, sung2018learning} and optimization-based meta-learning \cite{ravi2016optimization, finn2017model, rusu2018meta, nichol2018first}.
% Recently, \cite{tian2020rethinking, dhillon2020baseline, chen2019closer} showed that training a classifier upon a good representation is on par with multiple previous works employing meta-learning. 
% Inspired by these works, we avoid the use of meta-learning and we use the standard procedure to train a network on the base classes. However, differently from them we perform and end-to-end training when learning the novel classes, showing that it is beneficial to improve performance.
% }

\myparagraph{Few-Shot Learning} is often considered as a binary %Multiple works considered the few-shot learning 
problem in semantic segmentation, % as a binary problem, 
where the goal is to learn to segment a novel class given only few images %the few-shot learning scenario has been extended to semantic segmentation, where different works have been proposed 
\cite{shaban2017one, rakelly2018few, dong2018few, zhang2019canet, wang2019panet, siam2019adaptive}. Few methods extended the analysis on multiple classes \cite{dong2018few, wang2019panet, zhang2020sg}, but limiting the evaluation to as few as 2 new classes.
To overcome these limitations, \cite{xian2019spnet} proposed the Generalized Few-Shot Segmentation setting, where the goal is to segment both base and new classes, learning them from several and few images respectively.
However, \cite{xian2019spnet} considers an offline scenario, assuming there is always access to a large dataset with annotations for old classes. % when learning new ones from few images.
In \SET\ we %want to % these approaches, we consider a multi-class problem in the incremental scenario. Our goal is to 
still extend a model with new classes given few images but \textit{without} access to previous datasets. While %e note that 
similar benchmarks %incremental few-shot learning benchmarks 
exist in image classification \cite{gidaris2018dynamic, tao2020few, ren2019incremental} and object detection \cite{perez2020incremental}, we are the first to study this setting in semantic segmentation. 

Finally, \ours\ is related to %few-shot classification 
methods \cite{tian2020rethinking, dhillon2020baseline, chen2019closer} training a randomly initialized classifier on new classes. % upon a good initial representation. % is very effective in few-shot settings. %on par with more complex meta-learning  employing meta-learning. 
%Inspired by these works, we also fine-tune %avoid the use of meta-learning and we use the standard procedure to train a network on the base classes. 
Unlike these methods,  %train only the classifier, randomly initializing it for novel classes,
we initialize the classifier of new classes using weight imprinting \cite{gidaris2018dynamic, qi2018low} and train the architecture end-to-end, with the help of a distillation loss to reduce overfitting. % over all classes. 
These differences significantly improve the performance on new classes. %representation of new classes, increasing the final performance by a margin.
%[here we may discuss paper on FSIL of CVPR 21 and FSIL in Instance seg.]

\myparagraph{Incremental Learning}
 aims to expand the output space of a model without forgetting old knowledge % in catastrophic forgetting 
\cite{mccloskey1989catastrophic}. %, \ie without %experiencing 
%a performance drop on old knowledge.
This problem has been extensively studied in image classification \cite{li2017learning,kirkpatrick2017overcoming,chaudhry2018riemannian,rebuffi2017icarl,hou2019learning,hou2019learning,yu2020semantic}, and %only recently in 
semantic segmentation \cite{ozdemir2019extending,michieli2019incremental,michieli2021knowledge,cermelli2020modeling, siam2019adaptive}.
While previous segmentation works add new classes from a large dataset, here we learn them from just few images.
%\fabio{[F: We need to cite also \cite{} as continual semantic segmentation setup and discuss differences]}.

Differently from distillation methods for IL % similar to IL methods 
\cite{michieli2019incremental,cermelli2020modeling,li2017learning}, \ours\ relies on prototype learning to % allows \ours\ uses a prototype-based classifier to 
effectively initialize the classifier of new classes, integrating them in the distillation loss to reduce both forgetting and overfitting. \fabio{Differently from \cite{siam2019adaptive}, we train of the whole network on the few-shot images using batch renormalization and knowledge distillation.} %and to overfitting 
%. %by including their prototypes in the distillation loss.


==> sec/supp_mat.tex <==
\section{Implementation details}
\vspace{10pt}
\subsection{Training protocol} \label{sec:training-protocol}
In this section, we provide additional details on the training protocol used in our experiments. Note that we adopt the same protocol for all the methods, to ensure a fair comparison. 

When fine-tuning we follow \cite{chen2018encoder}, using SGD as optimizer with momentum $0.9$, weight decay $10^{-4}$ and a polynomial learning rate policy, \ie $\text{lr} = \text{lr}_{\text{init}} (1- \frac{\text{iter}}{\max\_\text{iter}})^{0.9}$. 
During training, we apply the same data augmentation of \cite{chen2018encoder}, performing random scaling and horizontal flipping, % of the training images, 
with a crop-size of $512\times512$. While the previous hyperparameters are shared across settings, we use a different learning rate and number of training iterations depending on the dataset, number of shots and learning steps. In particular, in the base step we train the network for 30 epochs on Pascal-VOC and 20 epochs on COCO using learning rate $10^{-2}$ and batch size 24. For the FSL step t, we set the batch size to $\min(10, |\set D_t|)$. In the FSL steps of VOC-SS, we train for 1000 iterations with learning rate $10^{-3}$, and for 200 iterations per step for VOC-MS, with learning rate $10^{-4}$.
On COCO FSL steps we use a learning rate $10^{-3}$, training the model for 2000 iterations on COCO-SS, and 100 iterations on every step of COCO-MS. These training hyperparameters are shared by all methods.

\subsection{Adapting baselines to iFSS and hyperparameters choice}
In this section, we describe how we adapt the baselines reported in the main paper to iFSS and the value of their hyperparameters. We set the hyperparameters specific of each approach in the VOC-SS and COCO-SS 1-shot settings, using the first split of each dataset (\ie 5-0 for VOC, and 20-0 for COCO) and maintaining the same values across all other shots, splits and number of learning steps.

For Weight Imprinting (WI), we adapted the work of \cite{qi2018low} from image classification. In particular, we %as described in Sec.~4.1 of the main paper.
replaced the image-level feature extractor of \cite{qi2018low} with masked average pooling (MAP), as described in Sec.~4.1 of the paper. This method does not require additional hyperparameters, and we initialize the prototypes for new classes while keeping the prototypes of old ones unaltered. 

%\fabio{Come adattato su segm.}
Similarly, for Dynamic Weight Imprinting \cite{gidaris2018dynamic} (DWI), we implemented the classifier using the same attention mechanism and weight generator of \cite{gidaris2018dynamic}, but we replaced the class-specific image-level features with the ones extracted through MAP. DWI uses a second meta-learning training stage on the base classes {to refine the weight generator}. %In both stage we compute the loss (i.e. cross-entropy) pixel-wise instead of image-wise. 
We performed this step for $1000$ iterations, with learning rate $1.0$ and batch size 8, aggregating the gradient of 2 training episodes, as in~\cite{gidaris2018dynamic}. After the meta learning stage, the method includes new classes in the FSL steps by weight imprinting, that we implemented with MAP, as for WI.%  We underline that, since this method is not trained after the base step, the second learning stage has been performed once after the training on the base dataset.}

Rethinking FSL \cite{tian2020rethinking} (RT), refines the model during the base step by using self-distillation and fine-tunes the classifier on the FSL step. In particular, after the base step a copy of the model is stored and provides the target of the self-distillation loss, to the current model. This training phase uses the same hyperparameters of the base one. %after the base step the current model is saved performing multiple training rounds where the model is train the model in the base step with their self-distillation loss, applying it pixel-wise. \massi{
%after training the model in the base step, we perform another round of training, with the same hyperparameters of the base step but applying a self-distillation loss (pixel-wise), where the target are provided by a copy of the network at the end of the previous round. 
 We stopped after one additional training round %of self-distillation 
because we did not see clear improvements using more rounds at the expense of a longer training time. For iFSS, we applied the self-distillation loss pixel-wise.
For the FSL steps, we trained the classifier for new classes starting from random weights and freezing the rest of the network. We multiplied the learning rate by 10 \wrt the Sec~\ref{sec:training-protocol} on the FSL step, since this improved the performance on both datasets.

Adaptive Masked Proxies \cite{siam2019adaptive} (AMP) has been implemented following details in \cite{siam2019adaptive} uses a standard linear classification layer and, %following Eq.~1b of \cite{siam2019adaptive}, it uses 
an L2-normalized MAP features % of the features extracted with MAP 
as classifier for the new classes. 
% \massi{After initializing the weights of the new classes with normalized MAP, it continuously updates them if new images whenev normalizes the features obtained with masked average pooling. The classifier weights are updated following Eq.~2 of \cite{siam2019adaptive}, setting $\alpha$ equals to $0.25$. \fabio{Come adattato su vecchie.}}
We adapted AMP to work on both old and new classes using all the available annotations in the FSL dataset. In particular, as proposed by \cite{siam2019adaptive} for continuous segmentation, we update the classifier weights for all the old classes appearing in the new dataset by computing a moving average %, as in Eq.~2 of \cite{siam2019adaptive}, 
with update rate $\alpha=0.25$.

For Semantic Projection Network \cite{xian2019spnet} (SPN) we follow the implementation provided by the authors, using the combination of word2vec \cite{mikolov2013distributed} and fastText \cite{joulin2016fasttext} as class embeddings, using them direclty as classifier weights. %as in \cite{xian2019spnet}. 
The method has no specific hyperparameters and we adapt it to \SET\ by not retaining the old datasets in the learning steps.

We implemented the three incremental learning methods, Learning without Forgetting \cite{li2017learning} (LwF), Incremental Learning Techniques \cite{michieli2019incremental} (ILT), and Modeling the Background \cite{cermelli2020modeling} (MiB), following the code provided by \cite{cermelli2020modeling}. As regularizer, LwF and ILT apply a standard cross-entropy loss using the old network predictions as target, and ILT imposes an additional L2 constraint on the output of the backbone (\ie the Resnet-101). MiB uses the revised cross-entropy and distillation losses as well as the classifier weights initialization for new classes. The weight of the distillation losses is $100$ for LwF, $100$ on both the L2 and the cross-entropy for ILT, and $10$ for MiB. %For all methods, we use the few-shot images in place of the many-shots datasets of standard incremental learning. 

Finally, for our model we set $\lambda$ to $10$ for all settings. We recall that for all the baseline we report in the paper, we used the same training protocol and architectures of \ours. 

\begin{table}[t]
    \centering
    \begin{tabular}{c|p{5cm}}
         \textbf{split}  &  \textbf{classes} \\ \hline
         5-0  &  aeroplane, bicycle, bird, boat, bottle \\
         5-1  &  bus, car, cat, chair, cow \\
         5-2  &  table, dog, horse, motorbike, person \\
         5-3  &  plant, sheep, sofa, train, tv-monitor \\
    \end{tabular}
    \vspace{4pt}
    \caption{Pascal-VOC class split.} \label{tab:voc-split}
    \vspace{-4pt}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{p{1cm}|p{6.5cm}}
         \textbf{split}  &  \textbf{classes} \\ \hline
         20-0  &  person, airplane, boat, parking meter, dog, elephant, backpack, suitcase, sports ball, skateboard, wine glass, spoon, sandwich, hot dog, chair, dining table, mouse, microwave, refrigerator, scissors \\
         20-1  &  bicycle, bus, traffic light, bench, horse, bear, umbrella, frisbee, kite, surfboard, cup, bowl, orange, pizza, couch, toilet, remote, oven, book, teddy bear \\
         20-2  &  car, train, fire hydrant, bird, sheep, zebra, handbag, skis, baseball bat, tennis racket, fork, banana, broccoli, donut, potted plant, tv, keyboard, toaster, clock, hair drier \\
         20-3  &  motorcycle, truck, stop sign, cat, cow, giraffe, tie, snowboard, baseball glove, bottle, knife, apple, carrot, cake, bed, laptop, cell phone, sink, vase, toothbrush \\
    \end{tabular}
    \vspace{4pt}
    \caption{COCO class split.} \label{tab:coco-split}
    \vspace{-4pt}
\end{table}

\subsection{Dataset class splits}
We split both Pascal-VOC and COCO in 4 folds, following previous works in semantic segmentation \cite{nguyen2019feature, wang2019panet, zhang2019canet, shaban2017one, rakelly2018few}. Table \ref{tab:voc-split} reports the detailed class folds for Pascal-VOC, \rev{taken from \cite{shaban2017one},} and Table \ref{tab:coco-split} the ones for the COCO dataset, \rev{taken from \cite{nguyen2019feature}}.

\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{fig/rebuttal/VOC_perc.png}
        \caption{VOC} 
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{fig/rebuttal/COCO_perc.png}
        \caption{COCO} 
    \end{subfigure}
    \vspace{5pt} \caption{Percentage of images containing the old class in the 5-shot setting datasets. We note that class \textit{person} has class-ID 15 on VOC and 1 on COCO. The red line represents the median over all classes.}
    \label{fig:perc_img}
\end{figure}


\rev{
\section{Influence of old classes annotations in iFSS}
The few-shot learning steps (FSL) in our benchmark consider a dataset with 1, 2, or 5 images for each new class, {randomly} sampled from the set of images containing at least one pixel of that class, but \textit{without} imposing any constraint about the presence of old classes. However, differently from \cite{cermelli2020modeling}, the few-shot datasets provide annotation for all available pixels, both for new and old classes.
In this section, we first analyze the frequency with which old classes appears in few-shot learning steps, showing that they co-occurs rarely with new classes.
Then, we compare the results of the settings using (non-strict IL) and not using (strict IL) old classes annotations.

\subsection{Frequency of old classes in few-shot learning datasets}
Fig.\ref{fig:perc_img} reports the percentage of images per old class averaged on all folds of the 5-shot settings.
From the figure, we note that old classes rarely co-occur when learning new classes: the median is 1.56\% of images per old class on VOC and 2.1\% on COCO. The only exception is the \textit{person} class that frequently appears in the few-shot dataset: in 32\% of images in VOC and in 52\% in COCO. Moreover, we note that many classes never appear with new classes, both in VOC, such as classes 4 (\textit{boat}) and 10 (\textit{cow}), and in COCO, \eg classes 22 (\textit{bear}) and 23 (\textit{zebra}).

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{c|c|ccc|ccc|ccc||ccc|ccc|ccc}
    \multicolumn{2}{c|}{} & \multicolumn{9}{c||}{\textbf{VOC-SS}} & \multicolumn{9}{c}{\textbf{COCO-SS}}  \\
    \multicolumn{2}{c|}{} & \multicolumn{3}{c}{\textbf{1-shot}} & \multicolumn{3}{c}{\textbf{2-shot}} & \multicolumn{3}{c||}{\textbf{5-shot}} & \multicolumn{3}{c}{\textbf{1-shot}} & \multicolumn{3}{c}{\textbf{2-shot}} & \multicolumn{3}{c}{\textbf{5-shot}} \\ \hline
    Method & Strict & mIoU-B & mIoU-N	 & HM	 & mIoU-B & mIoU-N	 & HM & mIoU-B & mIoU-N	 & HM & mIoU-B & mIoU-N	 & HM	 & mIoU-B & mIoU-N	 & HM & mIoU-B & mIoU-N	 & HM  \\ \hline     \rowcolor{rowColor}
    FT               &        & 58.2 &	 9.7 & 16.6	& 59.1 &	19.6 &	29.5 &	55.8 & 29.5 &	38.6                        & 41.2&	 4.1&	 7.5&	41.5&	 7.3&	12.4&	41.6&	12.3 &	19.0 \\ 
    FT        	     & \cmark & 55.0 &	10.2 & 17.2	& 55.5 &	19.2 &	28.5 &	43.7 & 26.8 &	33.2                        & 35.3&	 4.5&	 8.0&	32.8&	 7.4&	12.1&	26.9&	11.1&	15.7 \\ \rowcolor{rowColor}
    WI \cite{qi2018low}              &        & \bb{62.6} &	15.4 & 24.8	& 63.2 &	19.2 &	29.4 &	63.2 & 21.7 &	32.3                    & \bb{43.8}&	 6.9&	11.9&	44.2&	 7.9&	13.5&	43.6&	 8.7 &	14.6 \\ 
    WI \cite{qi2018low}      	     & \cmark & \br{62.6} &	15.4 & 24.8	& 63.2 &	19.2 &	29.4 &	63.2 & 21.7 &	32.3                    & \br{43.8}&	 6.9&	11.9&	\br{44.2}&	 7.9&	13.5&	43.6&	 8.7 &	14.6 \\ \rowcolor{rowColor}
    SPN  \cite{xian2019spnet}              &        & 59.8 &	16.3 & 25.6	& 60.7 &	\bb{26.3} &	\bb{36.7} &	58.3 & \bb{33.4} &	42.4            & 43.5&	 6.7&	11.7&	43.7&	10.2&	16.5&	43.7&	\bb{15.6} &	\bb{22.9} \\ 
    SPN  \cite{xian2019spnet}      	     & \cmark & 56.3 &	16.4 & 25.4	& 57.0 &	25.3 &	35.1 &	48.6 & 30.2 &	37.3                        & 38.1&	 7.0&	11.8&	37.0&	10.4&	16.3&	33.2&	15.1 &	20.8 \\ \rowcolor{rowColor}
    MIB \cite{cermelli2020modeling}             &        & 61.0 &	 5.2 &  9.6	& \bb{63.5} &	12.6 &	21.1 &	\bb{64.9} & 28.1 &	39.2                & \bb{43.8}&	 3.5&	 6.5&	\bb{44.4}&	 6.0&	10.6&	\bb{44.7}&	11.9 &	18.8 \\ 
    MIB \cite{cermelli2020modeling}      	     & \cmark & 61.0 &	 6.0 & 11.0	& \br{63.5} &	13.7 &	22.5 &	\br{64.9} & 29.4 &	40.4                & \br{43.7}&	 4.2&	 7.7&	\br{44.2}&	 7.1&	12.3&	\br{44.4}&	13.8 &	21.1 \\ \rowcolor{rowColor}
    PIFS             &        & 60.8 &	\bb{18.5} & \bb{28.4}	& 60.5 &	\bb{26.3} &	\bb{36.7} &	60.0 & 33.2 &\bb{42.8}  & 40.8&	 \bb{8.2}&	\bb{13.6}&	40.9&	11.1&	\bb{17.5}&	42.8&	\bb{15.7} &	\bb{23.0} \\ 
    PIFS      	     & \cmark & 59.1 &	\br{18.2} & \br{27.9}	& 58.8 &	26.1 &	36.2 &	57.2 & 32.5 &	41.5            & 34.9&	 \br{8.9}&	14.2&	34.6&	11.7&	17.4&	32.6&	15.6 &	21.1 \\ 
    PIFS*	    & \cmark & 60.3 &	18.0 & 27.7	& 60.3 &	\br{26.3} &	\br{36.6} &	59.5 & \br{33.0} &	\br{42.5}       & 38.8&	 8.8&	\br{14.4}&   39.2&	\br{11.8}&	\br{18.1}&	38.4&	\br{16.1} &	\br{22.6} \\ 
    \end{tabular}}
    \vspace{-2pt} \caption{Performance in strict and non-strict incremental learning on single-step settings. In bold-red the best method in strict-IL scenario. In bold-blue, the best method in non strict-IL. PIFS* uses the revised classification loss proposed by MIB \cite{cermelli2020modeling}.} \label{tab:strict}
    \vspace{-15pt}
\end{table*}

\subsection{Comparison between iFSS in strict and non-strict settings}
Tab.~\ref{tab:strict} reports the comparison among the strict and non-strict setting of some indicative methods, FT, WI \cite{qi2018low}, SPN \cite{xian2019spnet}, MIB \cite{cermelli2020modeling} and PIFS, evaluating the impact of the background shift on them. We also report PIFS*, which uses the revised classification loss proposed by MIB \cite{cermelli2020modeling} to deal with the background shift.
First, we note that WI obtains the same results in the two settings since it is not affected by the annotation on old classes and it only uses new classes' pixels for generating the classifier weights. 
Differently, FT and SPN, suffer the background shift, as indicated by the large decrease in mIoU-B on all setting. 
MIB, being designed to solve deal with the background shift, even improves its performance, obtaining similar results in mIoU-B and improving its performance on mIoU-N. 
Finally, we note that PIFS is robust to the background shift on VOC but it decrease in performance on mIoU-B on COCO. Moreover, it obtains outstanding performance on new classes, constantly outperforming the competitors on mIoU-N.
Introducing the cross-entropy loss of MiB \cite{cermelli2020modeling} in PIFS, it notably improves the results on old classes, alleviating the background shift. We remark that introducing the loss of \cite{cermelli2020modeling} is straightforward, since the choice of classification loss is independent from the prototype-learning and the distillation loss of PIFS.
}

\begin{figure}
  \centering
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{fig/plot22/voc1.pdf}
  \caption{VOC 1-shot}
  \vspace{-5pt}
\end{subfigure}%
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\textwidth]{fig/plot22/voc2.pdf}
  \caption{VOC 2-shot}
    \vspace{-5pt}
\end{subfigure}%
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\textwidth]{fig/plot22/voc5.pdf}
  \caption{VOC 5-shot}
    \vspace{-5pt}
\end{subfigure}
\begin{subfigure}{0.056\textwidth}
  \centering
  \includegraphics[width=\textwidth]{fig/plot22/legend.pdf}
    \vspace{2pt}
\end{subfigure}

\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\textwidth]{fig/plot22/coco1.pdf}
  \caption{COCO 1-shot}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\textwidth]{fig/plot22/coco2.pdf}
  \caption{COCO 2-shot}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\textwidth]{fig/plot22/coco5.pdf}
  \caption{COCO 5-shot}
\end{subfigure}
\begin{subfigure}{0.056\textwidth}
  \centering
  \includegraphics[width=\textwidth]{fig/plot22/legend.pdf}
  \vspace{2pt}
\end{subfigure}
\vspace{2pt}
\caption{\SET\ results on the sequential addition of new class. Every column is a new step.}
\vspace{-10pt}
\label{fig:multi-step}
\end{figure}

\section{Additional results}
\vspace{4pt}


\subsection{Detailed results step-by-step}
We report the results for every incremental step on the VOC-MS and COCO-MS settings in \figref{fig:multi-step}. For every incremental step, we report the harmonic mean (HM) between the mIoU on base ($\set C^0$) and new ($\set C^t \backslash \set C^0$) classes.

From the results, we note that fine-tuning (orange), RT \cite{chen2017rethinking} (green, circle), and incremental learning methods \cite{cermelli2020modeling, michieli2019incremental, li2017learning} (blue) obtain the worst performance on all settings. We argue that this is due to: i) not exploiting prototype learning, failing to correctly initialize and represent the new classes, and ii) not dealing with the non-\textit{i.i.d.} data, as demonstrated by the poor performances obtained on VOC when few images are provided (1- and 2-shot settings). 
On the other hand, methods that perform prototype learning, %do not perform training in the incremental steps, 
such as few-shot classification methods \cite{qi2018low, gidaris2018dynamic} (green) and AMP \cite{siam2019adaptive} (yellow, square), show a better trade-off between learning and forgetting. In particular, WI \cite{qi2018low} and DWI \cite{gidaris2018dynamic} achieve good performance on VOC, being close to \ours\ (red) especially on the 1-shot setting. However, we note that on VOC 5-shot and COCO, \ours\ obtains better performances since it fine-tunes the network on the few-shot data, obtaining a better representation while avoiding overfitting. AMP \cite{siam2019adaptive}, differently, is outperformed by \ours, remarking that it is essential to update the network representation and not only the prototypes during the FSL steps.
Finally, SPN \cite{xian2019spnet} (yellow, triangle) achieves good performance on the initial steps of COCO-MS 2- and 5-shot settings, even surpassing \ours. However, after only one (5-shot) or two (2-shot) learning steps its performances degrade and it is surpassed by \ours. This demonstrates that \ours\ improves the representation for new class pixels while better dealing with forgetting and non-\textit{i.i.d.} data, even without using external knowledge.
Overall, \ours\ is consistently the best on every dataset and shot.

\subsection{Detailed results for each split}
Due to space constraints, in the main paper we report the average results across the 4 splits of classes of each dataset. % in which we split the two datasets. % classes. 
Here, we report the detailed results in all folds separately, measuring them as the mIoU on base (\textit{mIoU-B}) and new (\textit{mIoU-N}) classes, and their harmonic mean (\textit{HM}). %Table \ref{tab:voc-split} reports the class folds for Pascal-VOC, and Table \ref{tab:coco-split} the ones for the COCO dataset. 


\myparagraph{Pascal VOC.} We report the results for Pascal-VOC with only one few-shot learning step (VOC-SS) on Tab.~\ref{tab:voc-ss-1} for 1-shot, on Tab.~\ref{tab:voc-ss-2} for 2-shot, and on Tab.~\ref{tab:voc-ss-5} for 5-shot. The results on each fold are consistent with their average. %, with 
%From the tables we can see that 
\ours\  is effective on all the VOC folds, being always the best on 1-shot, and always the best or second best on 2-shot scenario, in terms of HM. Moreover, we note that SPN is the second best on both 2-shot and 5-shot scenarios, on all folds.
On 5-shot scenario incremental learning methods become competitive to \ours, being ILT the best on 5-0 ($+1.7$\% HM \wrt \ours) and LwF on 5-1 ($+3.4$\% HM \wrt \ours). However the improvement of these methods is not consistent in other folds (\eg 5-3, where \ours\ improves ILT of 5.1\% in HM), %or settings (\ie 1-shot and 2-shot), 
obtaining an average performance lower than \ours. %  and SPN. 

Tables \ref{tab:voc-ms-1}, \ref{tab:voc-ms-2}, and \ref{tab:voc-ms-5} report the results (averaged per FSL step) for the multi step scenario (VOC-MS), for the 1, 2, and 5 shot respectively. We remark that this setting is particularly challenging since methods are provided only with 1, 2 or 5 images of the same class to train, resulting in very unbalanced and non-\textit{i.i.d} set. 
In this setting, \ours\ obtains the best results on 5-1, 5-2, and 5-3, in both 1, 2, and 5-shot setting, achieving the second best results on 5-0 on 2 and 5-shot. We note that methods obtaining excellent performance on VOC-SS struggle on this scenario. In particular, SPN performances are lower than \ours\ of 15\% HM on average, while incremental learning methods are not able to learn new classes properly, performing close to standard fine-tuning. %, \ie 30\% HM worse than \ours\ on average.
On the other hand, DWI and WI are effective on this scenario, since they can integrate new classes without forgetting previous knowledge. DWI is the second best method on both 1, 2, and 5-shot, being the best on the 5-0 fold. However, \ours\ still outperforms it by $0.5$\% HM on 1-shot, $2.1$\% HM on 2-shot, and $1.7$\% HM on 5-shot.

\myparagraph{COCO.} The results for COCO-SS are reported on tables \ref{tab:coco-ss-1} (1-shot), \ref{tab:coco-ss-2} (2-shot), and \ref{tab:coco-ss-5} (5-shots). From the tables we can see that \ours\ is consistently best or second best on every shot and fold. It achieves nearly 1\% HM more than the second best method in 1-shot ($13.6$\% \wrt DWI $12.8$\%) and in 2-shot ($17.5$\% \wrt SPN $16.5$\%). %We can see that this improvement is consistent across all the folds.
Differently, on 5-shot SPN achieves comparable performance to \ours, \ie $22.9$\% vs $23.0$ HM. From the detailed results on the folds we can see that while SPN obtains better results on 20-0 and 20-1 ($+1.0$\% HM and $+0.3$\% HM respectively), \ours\ outperforms it on 20-2 and 20-3 ($+0.5$\% and $+1.3$\% HM). % respectively). 

Finally, we report the results for COCO-MS on tables \ref{tab:coco-ms-1} (1-shot), \ref{tab:coco-ms-2} (2-shot), and \ref{tab:coco-ms-5} (5-shot). Also in this setting \ours\ is always the best or second best method across all shots and folds. In particular, it is the best on 1-shot on every fold, outperforming the second best method (DWI) by 1.3\% HM on average.
On the 2-shot setting, \ours\ is the best on 20-0 ($+1.8$\% HM \wrt SPN) and 20-1 ($+1.2$\% HM \wrt RT) folds, being second best on 20-2 ($-1.2$\% HM \wrt SPN) and 20-3 ($-0.8$\% HM \wrt SPN). Overall, \ours\ outperforms the second best method, SPN, by $0.6$\% HM.
In the 5-shot setting, the performance of \ours\ and SPN are on par, achieving very similar results for both old and new classes. In particular, comparing them on the different folds, we see that they maintain very close performances, \ie in terms of HM, $22.9$\% vs $23.3$\% on 20-0, $22.3$\% vs $21.5$\% on 20-1, $26.4$\% vs $26.5$\% on 20-2, $29.5$\% vs $29.4$\% on 20-3, respectively for \ours\  and SPN.

\subsection{Prototype learning offline performance}
An open question from our results is whether prototype learning in the base step hampers the performance of the pretrained segmentation network. Ideally, we would like the model to retain the performance of a standard semantic segmentation model when trained offline, while keeping the advantage of prototype learning for the FSL steps.  

In this section, we show that prototype learning performs on par to other learning techniques in a standard offline setting, \ie when all the classes are learned in one step. To demonstrate this, in Tab.~\ref{tab:off-results} we report the results for a linear classifier trained with cross-entropy (std), SPN \cite{xian2019spnet}, and \ours\   %prototype learning 
on the base step of COCO. 
From the results we can see that our model is competitive with both choices, achieving an average mIoU of 52.1\% vs 53.0\% of SPN and 52.9\% of standard training. %is  \ours\ is competitive with both choices.slightly better than standard training ($0.1$\% mIoU) and \ours\  ($0.9$\% mIoU). However, we can note that \ours\  is competitive with both choices.  Moreover, we 
Note that while \ours\ performs comparably to other approaches in the offline scenario, the improvement on the incremental few-shot learning settings is remarkable, as demonstrated in previous experiments.

\subsection{Additional qualitative results}
Due to space constraints, in the paper we report only the qualitative results for VOC-SS 1-shot. Here, we expand the analysis by reporting the results for other scenarios, \ie COCO-SS 1-shot, COCO-SS 2-shot and VOC-SS 2-shot. %dataset and extending the analysis also to the 2-shot scenario.

Fig.~\ref{fig:qualitative-coco} shows some qualitative results for different methods on COCO-SS 1-shot. From the figure, we can see how \ours\ better discriminates the new class \wrt other approaches. Overall, we see that WI and DWI tend to assign pixels to new classes even when they are outside the class of interest (\eg \textit{dog} second row, \textit{wc}, fourth row), while ILT and SPN may either ignore pixels of new classes (\eg \textit{surfboard} third row) or assign them to old ones (\eg \textit{elephant} first row). On the other hand, \ours\ correctly segments both old and new classes, even in images with clutter (\eg \textit{surfboard} third row), multiple instances (\eg \textit{sheep} last row) and complex boundaries (\eg \textit{dog} second row).

In Fig.~\ref{fig:qualitative-voc2} and Fig.~\ref{fig:qualitative-coco2} we show results for the VOC-SS and COCO-SS 2-shot settings. Similarly to VOC-SS 1-shot and COCO-SS 1-shot, non-finetuned methods (WI, DWI) may not discriminate new classes, %making incoherent prediction 
when they are similar to base ones, making incoherent predictions. Examples are \textit{cow} and \textit{bus} (first and second rows of \figref{fig:qualitative-voc2}) mistakenly segmented as \textit{horse} (purple) and \textit{train} (light-green) respectively,  and \textit{giraffe} (fifth row of \figref{fig:qualitative-coco2}) segmented as \textit{zebra} (blue). SPN and ILT may not properly learn to segment new classes when trained with few complex examples. For instance, both methods fail to segment \textit{motorcycle} (third row \figref{fig:qualitative-voc2}) and \textit{sofa} (\figref{fig:qualitative-coco2}, fourth row), where training images are either small and in cluttered environments (\eg \textit{motorcycle}) or mixed with other classes (\eg \textit{dogs} in \textit{sofa}). In contrast, \ours\ precisely segments new classes, discriminating them from old ones. For instance, our model correctly segments the multiple instances of \textit{motorcycle} and \textit{sheep} (last row) in \figref{fig:qualitative-voc2}, while separating pixels of \textit{cat} and \textit{dog} from the new class \textit{sofa} in \figref{fig:qualitative-coco2}. Interestingly, \ours\ can correctly discriminate almost all pixels of the new classes (\eg \textit{cow}, second row of \figref{fig:qualitative-voc2}, \textit{bear} and {\textit{sandwich}} in \figref{fig:qualitative-coco2} second and third rows), despite their similarities (\eg \textit{cow} with \textit{horse}) or large difference (\eg \textit{bear}) with old ones, or the presence of multiple other classes (\eg \textit{sandwich}).


\begin{table}[t]
    \centering
    \begin{tabular}{l|c||c|c|c|c}
         Method  &  Mean  &  20-0  &  20-1  &  20-2  &  20-3 \\ \hline
         std  &           52.9 & 			\textbf{49.8} & 			52.6 & 			\textbf{55.1} & 			54.2 \\
         SPN \cite{xian2019spnet}   &      \textbf{53.0} & 			49.5 & 			\textbf{53.2} & 			54.7 & 			\textbf{54.6} \\
         \ours             &  52.1 & 			47.9 & 			51.6 & 			54.4 & 			54.3 \\
    \end{tabular}
    \vspace{4pt}
    \caption{mIoU on base classes, before the few-shot steps, comparing the Prototype Learning (\ours) with a standard classifier (std) and SPN \cite{xian2019spnet} on the COCO dataset.} \label{tab:off-results}
\end{table}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{5-0}}  &  \multicolumn{3}{c|}{\textbf{5-1}}  &  \multicolumn{3}{c|}{\textbf{5-2}}  &  \multicolumn{3}{c}{\textbf{5-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  58.3 & 9.7 & 16.7 & 61.9 & 3.2 & 6.1 & 55.2 & 16.3 & 25.2 & 53.6 & 13.1 & 21.1 & 62.4 & 6.3 & 11.5 \\ \hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  62.7 & 15.5 & 24.8 & 66.5 & 10.5 & 18.1 & 58.9 & 21.9 & 31.9 & 58.6 & 15.3 & 24.2 & 66.7 & 14.2 & 23.5 \\
 &  DWI \cite{gidaris2018dynamic}       &  64.3 & 15.4 & 24.8 & 67.3 & 10.3 & 17.9 & 59.9 & 23.3 & \underline{33.5} & 60.0 & 16.0 & 25.3 & 69.9 & 11.8 & 20.2 \\
 &  RT \cite{tian2020rethinking}        &  59.1 & 12.1 & 20.1 & 62.7 & 3.8 & 7.1 & 54.5 & 18.7 & 27.9 & 56.3 & 14.6 & 23.2 & 63.1 & 11.4 & 19.3 \\ \hline
 \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  57.5 & 16.7 & \underline{25.8} & 61.7 & 12.0 & \underline{20.1} & 49.8 & 22.9 & 31.4 & 54.8 & 15.3 & 23.9 & 63.5 & 16.5 & \textbf{26.1} \\
 &  SPN  \cite{xian2019spnet}           &  59.8 & 16.3 & 25.6 & 64.1 & 9.0 & 15.8 & 56.2 & 23.9 & \underline{33.5} & 56.2 & 19.3 &\underline{ 28.7} & 62.7 & 13.1 & 21.7 \\ \hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  61.5 & 10.7 & 18.2 & 63.7 & 2.8 & 5.3 & 59.0 & 19.3 & 29.0 & 59.1 & 14.1 & 22.8 & 64.0 & 6.6 & 11.9 \\
 &  ILT  \cite{michieli2019incremental} &  64.3 & 13.6 & 22.5 & 67.1 & 5.9 & 10.8 & 60.5 & 19.3 & 29.2 & 61.2 & 18.9 & 28.9 & 68.4 & 10.3 & 18.0 \\
 &  MiB  \cite{cermelli2020modeling}    &  61.0 & 5.2 & 9.7 & 64.6 & 3.1 & 6.0 & 56.9 & 7.6 & 13.4 & 57.3 & 6.3 & 11.4 & 65.4 & 3.9 & 7.4 \\ \hline
 &  \textbf{\ours}                      &  60.9 & 18.6 & \textbf{28.4} & 64.4 & 12.7 & \textbf{21.2} & 54.3 & 25.1 & \textbf{34.3} & 57.1 & 20.3 & \textbf{29.9} & 67.6 & 16.2 & \textbf{26.1} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: VOC-SS 1-shot.} \label{tab:voc-ss-1}
    \vspace{-4pt}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{5-0}}  &  \multicolumn{3}{c|}{\textbf{5-1}}  &  \multicolumn{3}{c|}{\textbf{5-2}}  &  \multicolumn{3}{c}{\textbf{5-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  59.1 & 	19.7 & 	29.5 & 	61.7 & 	12.6 & 	20.9 & 	57.5 & 	31.0 & 	40.3 & 	54.8 & 	20.2 & 	29.5 & 	62.5 & 	15.0 & 	24.2 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  63.3 & 	19.2 & 	29.5 & 	67.1 & 	13.1 & 	21.9 & 	59.0 & 	28.2 & 	38.2 & 	59.3 & 	18.1 & 	27.7 & 	67.7 & 	17.5 & 	27.8 \\
 &  DWI \cite{gidaris2018dynamic}       &  64.8 & 	19.8 & 	30.4 & 	68.2 & 	15.1 & 	24.7 & 	60.4 & 	30.9 & 	40.9 & 	60.4 & 	17.2 & 	26.8 & 	70.1 & 	16.2 & 	26.3 \\
 &  RT \cite{tian2020rethinking}        &  60.9 & 	21.6 & 	31.9 & 	65.3 & 	10.4 & 	18.0 & 	54.4 & 	34.6 & 	42.3 & 	59.2 & 	24.3 & 	34.5 & 	64.7 & 	17.0 & 	27.0 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  54.4 & 	18.8 & 	27.9 & 	59.7 & 	12.5 & 	20.7 & 	44.5 & 	28.4 & 	34.7 & 	53.4 & 	17.2 & 	26.0 & 	59.8 & 	17.0 & 	26.5 \\
 &  SPN  \cite{xian2019spnet}           &  60.8 & 	26.3 & 	\underline{36.7 }& 	65.5 & 	18.8 & \textbf{	29.2} & 	57.1 & 	37.4 & 	\textbf{45.2} & 	57.8 & 	25.6 & \underline{	35.5} & 	62.7 & 	23.4 & 	\underline{34.1} \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  63.6 & 	18.9 & 	29.2 & 	65.2 & 	10.8 & 	18.6 & 	61.8 & 	31.3 & 	41.6 & 	60.9 & 	21.0 & 	31.3 & 	66.5 & 	12.6 & 	21.2 \\
 &  ILT  \cite{michieli2019incremental} &  64.2 & 	23.1 & 	34.0 & 	68.4 & 	16.1 & 	26.1 & 	58.3 & 	33.7 & 	42.7 & 	61.1 & 	25.6 & 	36.1 & 	68.9 & 	17.1 & 	27.4 \\
 &  MiB  \cite{cermelli2020modeling}    &  63.5 & 	12.7 & 	21.1 & 	66.6 & 	12.3 & 	20.7 & 	60.1 & 	18.3 & 	28.0 & 	59.7 & 	11.2 & 	18.8 & 	67.7 & 	9.0 & 	15.8 \\ \hline
 &  \textbf{\ours}                      &  60.5 & 	26.4 & 	\textbf{36.8} & 	64.0 & 	18.9 & 	\underline{29.1} & 	53.9 & 	36.6 & 	\underline{43.6} & 	58.2 & 	26.5 & 	\textbf{36.4} & 	65.9 & 	23.6 & \textbf{	34.7} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: VOC-SS 2-shot.} \label{tab:voc-ss-2}
    \vspace{-4pt}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{5-0}}  &  \multicolumn{3}{c|}{\textbf{5-1}}  &  \multicolumn{3}{c|}{\textbf{5-2}}  &  \multicolumn{3}{c}{\textbf{5-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  55.8 & 	29.6 & 	38.7 & 	58.4 & 	22.8 & 	32.8 & 	52.3 & 	42.7 & 	47.0 & 	50.6 & 	29.7 & 	37.5 & 	62.0 & 	23.0 & 	33.6 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  63.3 & 	21.7 & 	32.3 & 	67.5 & 	16.3 & 	26.3 & 	58.7 & 	30.8 & 	40.4 & 	59.4 & 	21.3 & 	31.4 & 	67.5 & 	18.4 & 	28.9 \\
 &  DWI \cite{gidaris2018dynamic}       &  64.9 & 	23.5 & 	34.5 & 	68.8 & 	20.7 & 	31.8 & 	60.8 & 	34.7 & 	44.2 & 	60.9 & 	20.6 & 	30.7 & 	69.1 & 	17.9 & 	28.5 \\
 &  RT \cite{tian2020rethinking}        &  60.4 & 	27.5 & 	37.8 & 	65.6 & 	19.1 & 	29.6 & 	55.8 & 	38.8 & 	45.8 & 	55.1 & 	29.3 & 	38.3 & 	65.0 & 	22.9 & 	33.9 \\ \hline
 \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  51.9 & 	18.9 & 	27.7 & 	58.5 & 	12.9 & 	21.2 & 	38.5 & 	26.5 & 	31.4 & 	51.9 & 	20.4 & 	29.3 & 	58.5 & 	15.8 & 	24.8 \\
 &  SPN  \cite{xian2019spnet}           &  58.4 & 	33.4 & 	\underline{42.5} & 	63.3 & 	28.2 & 	\underline{39.0 }& 	53.4 & 	43.7 & 	\underline{48.1} & 	54.5 & 	33.5 & 	41.5 & 	62.3 & 	28.2 & 	\underline{38.8} \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  59.7 & 	30.9 & 	40.8 & 	62.8 & 	23.9 & 	34.6 & 	57.1 & 	44.0 & 	\textbf{49.7} & 	55.9 & 	31.6 & 	40.3 & 	63.0 & 	24.4 & 	35.2 \\
 &  ILT  \cite{michieli2019incremental} &  61.4 & 	32.0 & 	42.1 & 	67.2 & 	27.8 & 	\textbf{39.4} & 	54.2 & 	40.4 & 	46.3 & 	57.1 & 	33.8 & 	\underline{42.4} & 	67.0 & 	26.1 & 	37.5 \\
 &  MiB  \cite{cermelli2020modeling}    &  65.0 & 	28.1 & 	39.3 & 	68.0 & 	24.8 & 	36.4 & 	62.1 & 	35.2 & 	44.9 & 	60.6 & 	27.1 & 	37.4 & 	69.1 & 	25.4 & 	37.2 \\ \hline
 &  \textbf{\ours}                      &  60.0 & 	33.3 & 	\textbf{42.8 }& 	64.3 & 	26.7 & 	37.7 & 	53.3 & 	41.0 & 	46.3 & 	57.4 & 	33.8 & \textbf{	42.5} & 	65.2 & 	31.6 & \textbf{42.6} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: VOC-SS 5-shot.} \label{tab:voc-ss-5}
    \vspace{-4pt}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{5-0}}  &  \multicolumn{3}{c|}{\textbf{5-1}}  &  \multicolumn{3}{c|}{\textbf{5-2}}  &  \multicolumn{3}{c}{\textbf{5-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  47.2 & 	3.9 & 	7.2 & 	46.8 & 	2.0 & 	3.8 & 	42.0 & 	8.0 & 	13.4 & 	47.3 & 	3.5 & 	6.5 & 	52.7 & 	2.1 & 	4.0 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  66.6 & 	16.1 & 	25.9 & 	68.8 & 	14.9 & 	\underline{24.5} & 	63.5 & 	24.4 & 	35.3 & 	63.3 & 	14.3 & 	\underline{23.4} & 	70.9 & 	10.6 & 	18.5 \\
 &  DWI \cite{gidaris2018dynamic}       &  67.2 & 	16.3 & \underline{26.2} & 69.0 & 15.7 & \textbf{25.6} & 63.6 & 25.8 & \underline{36.7} & 64.1 & 13.6 & 22.5 & 71.9 & 10.0 & 17.6 \\
 &  RT \cite{tian2020rethinking}        &  49.2 & 5.8 & 10.4 & 45.4 & 2.2 & 4.2 & 41.5 & 12.4 & 19.1 & 46.7 & 4.8 & 8.6 & 53.3 & 4.5 & 8.2 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  58.6 & 14.5 & 23.2 & 61.6 & 12.1 & 20.2 & 54.5 & 22.8 & 32.1 & 56.1 & 11.8 & 19.5 & 62.4 & 11.3 &\underline{ 19.1} \\
 &  SPN  \cite{xian2019spnet}           &  49.8 & 8.1 & 13.9 & 48.7 & 3.6 & 6.6 & 44.0 & 13.7 & 20.9 & 51.4 & 8.7 & 14.9 & 55.0 & 6.5 & 11.7 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  42.1 & 3.3 & 6.2 & 42.1 & 1.8 & 3.4 & 37.9 & 6.8 & 11.5 & 41.4 & 2.5 & 4.7 & 47.1 & 2.2 & 4.3 \\
 &  ILT  \cite{michieli2019incremental} &  43.7 & 3.3 & 6.1 & 42.3 & 1.7 & 3.3 & 41.0 & 6.1 & 10.6 & 41.9 & 3.5 & 6.4 & 49.6 & 1.8 & 3.4 \\
 &  MiB  \cite{cermelli2020modeling}    &  43.9 & 2.6 & 4.9 & 41.0 & 1.0 & 2.0 & 40.2 & 5.8 & 10.2 & 43.4 & 2.4 & 4.5 & 51.0 & 1.1 & 2.2 \\ \hline
 &  \textbf{\ours}                      &  64.1 & 	16.9 & 	\textbf{26.7} & 	67.6 & 	13.3 & 	22.3 & 	58.0 & 	27.1 & 	\textbf{36.9} & 	61.0 & 	15.6 & 	\textbf{24.9} & 	69.8 & 	11.5 & 	\textbf{19.8} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: VOC-MS 1-shot.} \label{tab:voc-ms-1}
    \vspace{-4pt}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{5-0}}  &  \multicolumn{3}{c|}{\textbf{5-1}}  &  \multicolumn{3}{c|}{\textbf{5-2}}  &  \multicolumn{3}{c}{\textbf{5-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  53.5 & 4.4 & 8.1 & 54.5 & 2.3 & 4.5 & 51.2 & 8.9 & 15.2 & 51.5 & 4.3 & 7.9 & 56.9 & 2.2 & 4.3 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  66.6 & 19.8 & 30.5 & 69.1 & 17.1 & 27.4 & 63.7 & 31.9 & 42.5 & 63.5 & 16.7 & \underline{26.5} & 70.3 & 13.5 & 22.7 \\
 &  DWI \cite{gidaris2018dynamic}       &  67.5 & 21.6 & \underline{32.7} & 69.7 & 21.3 & \textbf{32.6} & 63.9 & 35.4 & \underline{45.6} & 64.3 & 15.8 & 25.4 & 72.0 & 14.0 & \underline{23.5} \\
 &  RT \cite{tian2020rethinking}        &  36.0 & 4.9 & 8.6 & 43.8 & 3.1 & 5.8 & 23.0 & 7.2 & 11.0 & 28.3 & 5.3 & 9.0 & 40.7 & 4.7 & 8.5 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  58.4 & 16.3 & 25.5 & 62.3 & 12.3 & 20.6 & 54.0 & 27.2 & 36.1 & 55.9 & 14.7 & 23.3 & 61.5 & 10.8 & 18.4 \\
 &  SPN  \cite{xian2019spnet}           &  56.4 & 10.4 & 17.6 & 58.3 & 5.8 & 10.6 & 54.0 & 18.2 & 27.2 & 55.6 & 10.4 & 17.5 & 57.8 & 7.3 & 13.0 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  51.6 & 3.9 & 7.3 & 50.7 & 1.9 & 3.7 & 49.4 & 8.6 & 14.7 & 50.4 & 3.4 & 6.3 & 55.9 & 1.7 & 3.4 \\
 &  ILT  \cite{michieli2019incremental} &  52.2 & 4.4 & 8.1 & 50.7 & 2.0 & 3.9 & 51.6 & 9.7 & 16.3 & 49.9 & 4.0 & 7.4 & 56.8 & 1.7 & 3.4 \\
 &  MiB  \cite{cermelli2020modeling}    &  51.9 & 2.1 & 4.0 & 52.7 & 1.7 & 3.4 & 47.9 & 3.4 & 6.4 & 50.6 & 2.5 & 4.7 & 56.4 & 0.8 & 1.5 \\ \hline
 &  \textbf{\ours}                      &  65.2 & 23.7 & \textbf{34.8} & 68.0 & 17.7 & \underline{28.1} & 61.3 & 40.4 & \textbf{48.7} & 62.5 & 21.8 & \textbf{32.4} & 69.2 & 15.0 & \textbf{24.7} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: VOC-MS 2-shot.} \label{tab:voc-ms-2}
    \vspace{-4pt}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{5-0}}  &  \multicolumn{3}{c|}{\textbf{5-1}}  &  \multicolumn{3}{c|}{\textbf{5-2}}  &  \multicolumn{3}{c}{\textbf{5-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  58.7 & 7.7 & 13.6 & 59.9 & 5.1 & 9.5 & 57.0 & 14.8 & 23.5 & 55.9 & 7.1 & 12.5 & 62.5 & 3.7 & 7.0 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  66.6 & 21.9 & 33.0 & 69.6 & 20.4 & 31.5 & 63.4 & 32.9 & 43.3 & 63.4 & 20.1 & \underline{30.6} & 69.9 & 14.3 & 23.8 \\
 &  DWI \cite{gidaris2018dynamic}       &  67.6 & 25.4 & \underline{36.9} & 70.3 & 27.9 & \textbf{39.9} & 64.1 & 38.0 & \underline{47.7} & 64.5 & 19.6 & 30.1 & 71.5 & 16.0 & \underline{26.1} \\
 &  RT \cite{tian2020rethinking}        &  45.1 & 10.0 & 16.4  & 52.5 & 7.3 & 12.7 & 35.4 & 16.7 & 22.7 & 39.4 & 9.3 & 15.0 & 53.1 & 6.9 & 12.2 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  57.1 & 17.2 & 26.4 & 62.5 & 13.5 & 22.2 & 50.1 & 25.3 & 33.7 & 55.1 & 18.7 & 28.0 & 60.8 & 11.2 & 18.9 \\
 &  SPN  \cite{xian2019spnet}           &  61.6 & 16.3 & 25.8 & 62.3 & 10.4 & 17.9 & 59.5 & 27.6 & 37.7 & 60.3 & 14.7 & 23.7 & 64.2 & 12.3 & 20.6 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  59.8 & 7.5 & 13.4 & 60.7 & 5.2 & 9.6 & 57.8 & 14.6 & 23.3 & 57.4 & 6.8 & 12.2 & 63.3 & 3.5 & 6.6 \\
 &  ILT  \cite{michieli2019incremental} &  59.0 & 7.9 & 13.9 & 59.9 & 5.4 & 9.8 & 57.0 & 15.0 & 23.8 & 56.0 & 7.1 & 12.6 & 62.9 & 4.0 & 7.6 \\
 &  MiB  \cite{cermelli2020modeling}    &  60.9 & 5.8 & 10.5 & 61.0 & 4.8 & 8.9 & 58.4 & 9.6 & 16.5 & 59.5 & 5.9 & 10.8 & 64.9 & 2.7 & 5.2 \\ \hline
 &  \textbf{\ours}                      &  64.5 & 27.5 & \textbf{38.6} & 67.4 & 23.8 & \underline{35.2} & 60.4 & 41.6 & \textbf{49.3} & 61.6 & 25.4 & \textbf{35.9} & 68.6 & 19.0 &\textbf{ 29.8} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: VOC-MS 5-shot.} \label{tab:voc-ms-5}
    \vspace{-4pt}
\end{table*}


\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{20-0}}  &  \multicolumn{3}{c|}{\textbf{20-1}}  &  \multicolumn{3}{c|}{\textbf{20-2}}  &  \multicolumn{3}{c}{\textbf{20-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  41.2 & 4.1 & 7.5 & 36.2 & 2.0 & 3.8 & 40.6 & 4.9 & 8.7 & 45.0 & 3.7 & 6.8 & 43.1 & 5.8 & 10.3 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  43.8 & 6.9 & 11.9 & 41.0 & 4.8 & 8.6 & 42.8 & 7.8 & 13.2 & 46.4 & 6.8 & 11.8 & 45.1 & 8.1 & 13.8 \\
 &  DWI \cite{gidaris2018dynamic}       &  44.5 & 7.5 & \underline{12.8} & 39.8 & 5.0 & \underline{8.9} & 44.4 & 8.2 & \underline{13.9} & 47.2 & 6.8 & 11.9 & 46.6 & 9.9 & \underline{16.4} \\
 &  RT \cite{tian2020rethinking}        &  46.2 & 5.8 & 10.2 & 39.4 & 3.4 & 6.2 & 46.5 & 6.1 & 10.8 & 50.4 & 5.3 & 9.6 & 48.4 & 8.2 & 14.1 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  37.5 & 7.4 & 12.4 & 33.4 & 4.8 & 8.4 & 37.4 & 8.4 & 13.8 & 39.9 & 8.7 & \textbf{14.2} & 39.1 & 7.8 & 13.0 \\
 &  SPN  \cite{xian2019spnet}           &  43.5 & 6.7 & 11.7 & 39.2 & 4.6 & 8.2 & 43.7 & 6.4 & 11.1 & 46.8 & 7.1 & 12.3 & 44.3 & 8.9 & 14.8 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  43.9 & 3.8 & 7.0 & 37.8 & 1.8 & 3.4 & 43.7 & 4.3 & 7.9 & 47.9 & 3.7 & 6.8 & 46.1 & 5.4 &  9.6 \\
 &  ILT  \cite{michieli2019incremental} &  46.2 & 4.4 & 8.0 & 40.7 & 2.4 & 4.5 & 46.0 & 4.4 & 8.1 & 50.3 & 4.7 & 8.6 & 47.8 & 6.0 & 10.6 \\
 &  MiB  \cite{cermelli2020modeling}    &  43.8 & 3.5 & 6.5 & 37.5 & 2.1 & 4.0 & 44.1 & 3.6 & 6.6 & 47.6 & 3.9 & 7.1 & 46.0 & 4.4 &  8.1  \\ \hline
 &  \textbf{\ours}                      &  40.8 & 8.2 & \textbf{13.6} & 38.6 & 5.4 & \textbf{9.5} & 39.7 & 8.6 & \textbf{14.2} & 43.5 & 7.7 & \underline{13.1} & 41.4 & 10.9 & \textbf{17.2} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: COCO-SS 1-shot.} \label{tab:coco-ss-1}
    \vspace{-4pt}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{20-0}}  &  \multicolumn{3}{c|}{\textbf{20-1}}  &  \multicolumn{3}{c|}{\textbf{20-2}}  &  \multicolumn{3}{c}{\textbf{20-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  41.5 & 7.3 & 12.4 & 37.4 & 4.2 & 7.6 & 40.3 & 9.0 & 14.7 & 45.4 & 7.7 & 13.2 & 43.1 & 8.4 & 14.0 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  44.2 & 7.9 & 13.5 & 41.8 & 5.2 & 9.2 & 43.3 & 9.8 & 16.0 & 46.8 & 7.6 & 13.1 & 44.7 & 9.2 & 15.3 \\
 &  DWI \cite{gidaris2018dynamic}       &  45.0 & 9.4 & 15.6 & 40.4 & 6.1 & 10.6 & 45.2 & 10.7 & 17.4 & 47.4 & 9.1 & 15.3 & 46.9 & 11.8 & \underline{18.8} \\
 &  RT \cite{tian2020rethinking}        &  46.7 & 8.8 & 14.8 & 40.6 & 5.5 & 9.7 & 46.8 & 10.5 & 17.2 & 50.8 & 8.1 & 14.0 & 48.5 & 11.1 & 18.1 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  35.7 & 8.8 & 14.2 & 30.9 & 5.8 & 9.8 & 36.2 & 10.5 & 16.3 & 38.4 & 9.2 & 14.8 & 37.3 & 9.9 & 15.6 \\
 &  SPN  \cite{xian2019spnet}           &  43.7 & 10.2 & \underline{16.5} & 40.0 & 6.7 & \underline{11.5} & 43.3 & 11.5 & \underline{18.1} & 47.0 & 10.7 & \underline{17.5} & 44.6 & 11.9 & 18.7 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  44.3 & 7.1 & 12.3 & 39.2 & 4.5 & 8.0 & 43.8 & 8.7 & 14.5 & 48.1 & 7.3 & 12.7 & 46.0 & 8.0 & 13.6 \\
 &  ILT  \cite{michieli2019incremental} &  46.3 & 6.5 & 11.5 & 40.5 & 4.5 & 8.1 & 46.3 & 7.1 & 12.3 & 50.4 & 6.7 & 11.8 & 48.1 & 7.9 & 13.5 \\
 &  MiB  \cite{cermelli2020modeling}    &  44.4 & 6.0 & 10.6 & 38.2 & 4.2 & 7.6 & 44.5 & 7.1 & 12.3 & 48.6 & 6.5 & 11.4 & 46.3 & 6.1 & 10.8 \\ \hline
 &  \textbf{\ours}                      &  40.9 & 11.1 & \textbf{17.5} & 38.6 & 6.8 & \textbf{11.6} & 39.4 & 13.1 & \textbf{19.7} & 43.5 & 11.4 &\textbf{ 18.1} & 42.2 & 13.1 &\textbf{ 20.0} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: COCO-SS 2-shot.} \label{tab:coco-ss-2}
    \vspace{-4pt}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{20-0}}  &  \multicolumn{3}{c|}{\textbf{20-1}}  &  \multicolumn{3}{c|}{\textbf{20-2}}  &  \multicolumn{3}{c}{\textbf{20-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  41.6 & 12.3 & 19.0 & 37.3 & 7.6 & 12.6 & 40.9 & 15.0 & 22.0 & 45.3 & 13.7 & 21.0 & 43.0 & 12.9 & 19.8 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  43.6 & 8.7 & 14.6 & 41.7 & 6.0 & 10.5 & 42.8 & 10.7 & 17.1 & 45.7 & 8.6 & 14.4 & 44.4 & 9.7 & 15.9 \\
 &  DWI \cite{gidaris2018dynamic}       &  44.9 & 12.1 & 19.1 & 40.5 & 8.2 & 13.6 & 45.3 & 14.4 & 21.9 & 47.0 & 12.2 & 19.4 & 46.7 & 13.7 & 21.2 \\
 &  RT \cite{tian2020rethinking}        &  46.9 & 13.7 & 21.2 & 41.1 & 9.5 & 15.4 & 46.4 & 15.9 & 23.7 & 50.7 & 13.8 & 21.6 & 49.1 & 15.7 & 23.8 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  34.6 & 11.0 & 16.7 & 31.2 & 7.2 & 11.6 & 34.8 & 14.5 & 20.4 & 36.9 & 10.9 & 16.8 & 35.6 & 11.5 & 17.4 \\
 &  SPN  \cite{xian2019spnet}           &  43.7 & 15.6 & \textbf{22.9} & 40.1 & 11.5 &\textbf{ 17.9} & 42.9 & 17.7 &\textbf{ 25.1} & 46.4 & 16.4 & \underline{24.2} & 45.4 & 16.6 & \underline{24.4} \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  44.6 & 12.9 & 20.1 & 39.6 & 8.0 & 13.3 & 43.7 & 15.9 & 23.3 & 48.6 & 14.1 & 21.9 & 46.4 & 13.8 & 21.2 \\
 &  ILT  \cite{michieli2019incremental} &  47.0 & 11.0 & 17.8 & 41.9 & 7.1 & 12.2 & 47.0 & 13.9 & 21.5 & 50.4 & 11.2 & 18.3 & 48.6 & 11.8 & 19.0 \\
 &  MiB  \cite{cermelli2020modeling}    &  44.7 & 11.9 & 18.8 & 38.2 & 8.1 & 13.4 & 44.9 & 13.9 & 21.2 & 49.0 & 13.4 & 21.0 & 46.7 & 12.2 & 19.3 \\ \hline
 &  \textbf{\ours}                      &  42.8 & 15.7 & \textbf{23.0} & 40.6 & 10.7 & \underline{16.9} & 41.5 & 17.7 & \underline{24.8} & 45.3 & 16.9 & \textbf{24.7} & 43.9 & 17.5 & \textbf{25.0} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: COCO-SS 5-shot.} \label{tab:coco-ss-5}
    \vspace{-4pt}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{20-0}}  &  \multicolumn{3}{c|}{\textbf{20-1}}  &  \multicolumn{3}{c|}{\textbf{20-2}}  &  \multicolumn{3}{c}{\textbf{20-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  38.5 & 4.8 & 8.6 & 33.3 & 3.8 & 6.8 & 39.8 & 3.6 & 6.6 & 40.3 & 4.1 & 7.5 & 40.5 & 7.8 & 13.1 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  46.3 & 8.3 & 14.0 & 42.6 & 5.6 & 9.9 & 45.9 & 9.1 & 15.2 & 48.9 & 8.1 & 13.8 & 47.9 & 10.3 & 17.0 \\
 &  DWI \cite{gidaris2018dynamic}       &  46.2 & 9.2 & \underline{15.3} & 41.0 & 5.7 & 9.9 & 46.5 & 9.7 & \textbf{16.0} & 48.8 & 8.6 &\underline{ 14.7} & 48.6 & 12.7 & \underline{20.1} \\
 &  RT \cite{tian2020rethinking}        &  38.4 & 5.2 & 9.1 & 34.4 & 2.5 & 4.6 & 42.2 & 5.7 & 10.1 & 45.1 & 6.0 & 10.6 & 31.8 & 6.4 & 10.7 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  36.6 & 7.9 & 13.1 & 34.0 & 6.7 & 11.2 & 36.7 & 8.0 & 13.2 & 38.5 & 8.2 & 13.6 & 37.2 & 8.8 & 14.2 \\
 &  SPN  \cite{xian2019spnet}           &  40.3 & 8.7 & 14.3 & 37.1 & 7.5 & \underline{12.4} & 41.1 & 7.0 & 11.9 & 42.3 & 8.2 & 13.7 & 40.6 & 12.2 & 18.8 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  41.0 & 4.1 & 7.4 & 35.5 & 3.3 & 6.0 & 42.4 & 2.7 & 5.2 & 42.9 & 3.8 & 6.9 & 43.1 & 6.6 & 11.4 \\
 &  ILT  \cite{michieli2019incremental} &  43.7 & 6.2 & 10.8 & 38.5 & 4.8 & 8.5 & 45.0 & 4.8 & 8.7 & 45.8 & 5.2 & 9.4 & 45.5 & 10.0 & 16.4 \\
 &  MiB  \cite{cermelli2020modeling}    &  40.4 & 3.1 & 5.8 & 32.8 & 1.2 & 2.4 & 41.5 & 2.3 & 4.4 & 43.9 & 3.9 & 7.1 & 43.4 & 5.0 & 9.0 \\ \hline
 &  \textbf{\ours}                      &  40.4 & 10.4 & \textbf{16.6} & 37.0 & 8.3 & \textbf{13.6} & 40.5 & 10.0 & \textbf{16.0 }& 42.0 & 9.1 & \textbf{15.0} & 42.3 & 14.3 & \textbf{21.4} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: COCO-MS 1-shot.} \label{tab:coco-ms-1}
    \vspace{-4pt}
\end{table*}
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{20-0}}  &  \multicolumn{3}{c|}{\textbf{20-1}}  &  \multicolumn{3}{c|}{\textbf{20-2}}  &  \multicolumn{3}{c}{\textbf{20-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  40.3 & 6.8 & 11.7 & 36.4 & 5.5 & 9.5 & 40.4 & 5.1 & 9.0 & 42.5 & 6.0 & 10.6 & 41.8 & 10.8 & 17.1 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  46.5 & 9.3 & 15.4 & 43.2 & 5.8 & 10.3 & 46.1 & 10.0 & 16.4 & 49.1 & 9.5 & 15.9 & 47.5 & 11.7 & 18.8 \\
 &  DWI \cite{gidaris2018dynamic}       &  46.5 & 11.4 & 18.3 & 35.8 & 7.1 & 11.8 & 39.4 & 9.3 & 15.0 & 41.2 & 9.4 & 15.4 & 43.1 & 7.8 & 13.3 \\
 &  RT \cite{tian2020rethinking}        &  43.8 & 10.1 & 16.4 & 38.6 & 5.6 & 9.8 & 44.3 & 11.3 & \underline{18.0 }& 47.0 & 8.7 & 14.6 & 45.2 & 14.7 & 22.2 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  36.0 & 9.2 & 14.6 & 33.2 & 7.9 & 12.8 & 36.7 & 8.9 & 14.3 & 37.9 & 8.7 & 14.2 & 36.4 & 11.2 & 17.2 \\
 &  SPN  \cite{xian2019spnet}           &  41.7 & 12.5 & \underline{19.2} & 38.4 & 8.8 & \underline{14.3} & 41.9 & 10.1 & 16.3 & 44.0 & 13.6 & \textbf{20.8} & 42.5 & 17.3 & \textbf{24.6} \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  42.7 & 6.5 & 11.3 & 38.1 & 6.3 & 10.9 & 43.3 & 4.9 & 8.8 & 44.6 & 5.6 & 9.9 & 44.7 & 9.4 & 15.5 \\
 &  ILT  \cite{michieli2019incremental} &  47.1 & 10.0 & 16.5 & 46.5 & 7.1 & 12.3 & 48.5 & 8.0 & 13.7 & 47.7 & 13.2 & 20.7 & 45.7 & 11.9 & 18.8 \\
 &  MiB  \cite{cermelli2020modeling}    &  42.7 & 5.2 & 9.3 & 36.9 & 3.4 & 6.3 & 43.6 & 4.0 & 7.3 & 45.6 & 5.9 & 10.4 & 44.8 & 7.5 & 12.8 \\ \hline
 &  \textbf{\ours}                      &  40.1 & 13.1 & \textbf{19.8} & 37.2 & 10.3 & \textbf{16.1} & 39.9 & 12.7 & \textbf{19.2} & 42.4 & 12.7 & \underline{19.6} & 41.0 & 16.8 & \underline{23.8 }\\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: COCO-MS 2-shot.} \label{tab:coco-ms-2}
    \vspace{-4pt}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \resizebox{\linewidth}{!}
    {\begin{tabular}{ll|ccc||ccc|ccc|ccc|ccc}
     &    &   \multicolumn{3}{c||}{\textbf{Mean}}  &  \multicolumn{3}{c|}{\textbf{20-0}}  &  \multicolumn{3}{c|}{\textbf{20-1}}  &  \multicolumn{3}{c|}{\textbf{20-2}}  &  \multicolumn{3}{c}{\textbf{20-3}} \\ \hline
 &  Method	                          &  mIoU-B  &  mIoU-N	  &  HM	  &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM   &  mIoU-B  &  mIoU-N	  &  HM  &  mIoU-B  &  mIoU-N	  &  HM	  \\ \hline
 &  FT                                  &  39.5 & 11.5 & 17.8 & 36.1 & 11.1 & 17.0 & 38.4 & 9.3 & 15.0 & 42.0 & 10.6 & 16.9 & 41.5 & 14.8 & 21.8 \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FSC}}}
 &  WI \cite{qi2018low}                 &  46.3 & 10.3 & 16.8 & 43.4 & 7.3 & 12.4 & 45.7 & 11.1 & 17.8 & 48.7 & 10.5 & 17.2 & 47.4 & 12.3 & 19.5 \\
 &  DWI \cite{gidaris2018dynamic}       &  46.6 & 14.5 & 22.1 & 35.8 & 7.1 & 11.8 & 39.4 & 9.3 & 15.0 & 41.2 & 9.4 & 15.4 & 43.1 & 7.8 & 13.3 \\
 &  RT \cite{tian2020rethinking}        &  44.1 & 16.0 & 23.5 & 39.8 & 11.8 & 18.3 & 44.1 & 16.2 & \textbf{23.7 }& 47.0 & 15.7 & 23.6 & 45.4 & 20.2 & 28.0 \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FSS}}}
 &  AMP  \cite{siam2019adaptive}        &  33.2 & 11.0 & 16.5 & 30.8 & 9.3 & 14.2 & 33.5 & 11.6 & 17.3 & 34.5 & 10.2 & 15.8 & 34.0 & 12.9 & 18.7 \\
 &  SPN  \cite{xian2019spnet}           &  41.4 & 18.2 &\textbf{ 25.3} & 37.9 & 16.8 & \textbf{23.3} & 41.0 & 14.6 & 21.5 & 44.0 & 19.0 & \textbf{26.5 }& 42.8 & 22.4 & \underline{29.4} \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IL}}}
 &  LwF  \cite{li2017learning}          &  42.3 & 12.6 & 19.4 & 38.7 & 12.3 & 18.6 & 41.6 & 10.6 & 16.9 & 44.7 & 11.5 & 18.2 & 44.4 & 16.1 & 23.6 \\
 &  ILT  \cite{michieli2019incremental} &  45.3 & 15.3 & 22.8 & 41.1 & 14.5 & 21.4 & 45.3 & 13.7 & 21.0 & 47.8 & 14.1 & 21.8 & 47.1 & 18.8 & 26.9 \\
 &  MiB  \cite{cermelli2020modeling}    &  43.8 & 11.5 & 18.2 & 38.3 & 10.1 & 16.0 & 44.4 & 9.4 & 15.6 & 46.4 & 11.4 & 18.4 & 46.2 & 14.8 & 22.4 \\ \hline
 &  \textbf{\ours}                      &  41.1 & 18.3 &\textbf{ 25.3} & 38.2 & 16.3 & \underline{22.9} & 39.7 & 15.5 & \underline{22.3} & 43.7 & 18.9 & \underline{26.4} & 42.7 & 22.6 & \textbf{29.5} \\  

    \end{tabular}}
    \vspace{-4pt} \caption{\SET: COCO-MS 5-shot.} \label{tab:coco-ms-5}
    \vspace{-4pt}
\end{table*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/qual_coco.pdf}
    \vspace{-8pt}
    \caption{Qualitative results on the COCO-SS 1-shot setting.}
    \label{fig:qualitative-coco}
    \vspace{-4pt}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/qual_voc2.pdf}
    \vspace{-8pt}
    \caption{Qualitative results on the VOC-SS 2-shot setting.}
    \label{fig:qualitative-voc2}
    \vspace{-8pt}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/qual_coco2.pdf}
    \vspace{-8pt}
    \caption{Qualitative results on the COCO-SS 2-shot setting.}
    \label{fig:qualitative-coco2}
    \vspace{-8pt}
\end{figure*}



